Latent Diffusion Models with Masked AutoEncoders

In spite of the remarkable potential of Latent Diffusion Models (LDMs) in image generation, the desired properties and optimal design of the autoencoders have been underexplored. In this work, we analyze the role of autoencoders in LDMs and identify three key properties: latent smoothness, perceptual compression quality, and reconstruction quality. We demonstrate that existing autoencoders fail to simultaneously satisfy all three properties, and propose Variational Masked AutoEncoders (VMAEs), taking advantage of the hierarchical features maintained by Masked AutoEncoders. We integrate VMAEs into the LDM framework, introducing Latent Diffusion Models with Masked AutoEncoders (LDMAEs). Our code is available at https://github.com/isno0907/ldmae.

==> figures/class_uncurated_example2.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/mushroom947.drawio.png}
        \caption*{(a) Mushroom (947)}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/lakeside975.drawio.png}
        \caption*{(b) Lakeside (975)}
    \end{minipage}
    
    \vspace{0.5em} % 위아래 간격 조절
    
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/fig952.drawio.png}
        \caption*{(c) Fig (952)}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/vase883.drawio.png}
        \caption*{(d) Vase (883)}
    \end{minipage}

    \caption{\textbf{Uncurated Class-Conditional Generation on ImageNet-1K 2.} We present a collection of uncurated class-conditional images generated on ImageNet-1K at a resolution of $256\times256$. Each subcaption indicates the class name along with the corresponding class index.}
    \label{fig:uncurated2}
\end{figure*}


==> figures/silhouette_score.tex <==
\begin{figure}[t]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=.8\linewidth]{figures/images/silhouette_score.pdf}
    \vspace{-15pt}
    \caption{
        \textbf{Robustness of feature separation in latent space}. Our VMAEs show robust feature clustering consistently along the number of clusters, indicating strong feature separability. The scale is relative to the number of clusters at the semantic level.
    }
    \label{fig:silhouette}
    % \vspace{-0.3cm}
\end{figure}

==> figures/teaser_imagenet.tex <==
\begin{figure*}[t!]
    \centering
    % \includegraphics[width=0.9\textwidth]{figures/images/qualitative_comparison3.drawio.pdf}
    \includegraphics[width=\textwidth]{figures/images/qualitative_comparison_imagenet.drawio.png}
    % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \caption{\textbf{Vizualiation on ImageNet-1K ($256 \times 256$).} We visualize the images generated by our approach on the ImageNet-1K dataset.}
    % \caption{\textbf{Qualitative Results.} We visualize the generated images from our LDMAE on ImageNet 256x256 (top two rows) and CelebA-HQ 256x256 (bottom two rows). Our approach successfully captures the diversity and fine-grained details of natural images.}
    \label{fig:dm_teasor}
\end{figure*}


==> tables/ae_celebamask.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Perceptual-level segmentation on CelebAMask-HQ.} $\mu_{\text{intra}}$ and $\mu_{\text{inter}}$ denote the mean feature similarity of intra clusters and that of inter clusters, respectively.}
\resizebox{.8\columnwidth}{!}{%
\begin{tabular}{l|ccccc}
\toprule
\textbf{Model} & \textbf{AE} & \textbf{DAE} & \textbf{VAE}  & \textbf{SD-VAE}& \textbf{VMAE} \\
\midrule
$\mu_{\text{intra}} / \mu_{\text{inter}}$ & 1.646 & 1.832 & \textbf{3.044} & 1.270 & \underline{2.304}\\
\bottomrule
\end{tabular}%
}
\label{tab:ae_celebamask}
\end{table}







==> tables/ae_face_seg.tex <==
\begin{table}[t]
\centering
\caption{Feature separability in perceptual level evaluated on CelebAMask-HQ.}
\small
    \begin{tabular}{l|cc}
    \toprule
    \textbf{Model} & \textbf{gFID} $\downarrow$ & \textbf{sFID} $\downarrow$ \\
    \midrule
    AE & 24.80  & 29.90  \\
    DAE & - & - \\
    VAE & 43.90 & 54.59 \\
    SD3-VAE & 9.00 & 14.83 \\
    \textbf{MFAE (Ours)} & \textbf{8.59} & \textbf{12.32} \\
    \bottomrule
    \end{tabular}
\label{tab:face_seg}
\end{table}


==> tables/ae_separability.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Robustness of feature separation in latent space}. Our VMAEs show robust feature clustering consistently along the number of clusters, indicating strong feature separability. The scale is relative to the number of clusters at the semantic level.}
\resizebox{.9\columnwidth}{!}{
    \begin{tabular}{l|ccccc}
        \toprule
            &\multicolumn{5}{c}{\textbf{Number of Clusters}} \\ 
            \textbf{Model} & $\mathbf{1\times}$ & $\mathbf{2\times}$ & $\mathbf{3\times}$ & $\mathbf{4\times}$ & $\mathbf{5\times}$\\
        \midrule
            AE & 0.3518 & 0.1951& 0.0859&-0.0051&-0.0762\\
            DAE & \textbf{0.5102}&\textbf{0.3715}&\textbf{0.2542}&\underline{0.1491}&0.0579\\
            VAE & 0.2005&0.1846&0.1658&0.1442&\underline{0.1214}\\
            SD-VAE &0.2311&0.0693&-0.0496&-0.1313&-0.1884\\
            \textbf{VMAE (Ours)} & \underline{0.3129} & \underline{0.2771} & \underline{0.2397} & \textbf{0.2016} & \textbf{0.1643}\\
        \bottomrule
    \end{tabular}
}
\label{tab:silhouette}
\end{table}




% \begin{table}
%     \centering
%     \caption{\textbf{Normalized feature variance ($\sigma_F$) and similarity variance ($\sigma_S$).} MAE is trained for 800 epochs. All metrics are listed together with relative values to the MAE encoder.}
%     \vspace{-0.2cm}
%     % \resizebox{\linewidth}{!}{
%     \footnotesize{
%     \begin{tabular}{l|cc|cc} 
%             \toprule
%              & \multicolumn{2}{c|}{$\mathbb{E}[\sigma_F]$} & \multicolumn{2}{c}{$\mathbb{E}[\sigma_S]$} \\ 
%             % \midrule
%             Feature & Raw & Relative & Raw & Relative \\
%             \midrule
%             MAE encoder & 0.0008 & 1.00 & 0.075 & 1.00 \\ % Added more columns
%             MAE decoder & 0.0011 & 1.38 & 0.059 & 0.79 \\ % Added more columns
%             MOCO & 0.0001 & 0.15 & 0.003 & 0.05 \\ % Added more columns
%             ViT & 0.0002 & 0.32 & 0.012 & 0.16 \\ % Added more columns
%             %MAE fine-tuned & 0.0007 & 0.88 &  0.104 & 1.44\\ % Added more columns
%             \bottomrule
%     \end{tabular}
%     }
%     \vspace{-0.3cm}
%     \label{tab:mae_moco_vit}
% \end{table}

==> tables/celebahq_dm_table.tex <==
\begin{table}[t]
\centering
\caption{Performance comparison of unconditional generation in diffusion models using different autoencoders on CelebA-HQ ($256\times256$).}
\small
    \begin{tabular}{l|cc}
    \toprule
    \textbf{Model} & \textbf{gFID} $\downarrow$ & \textbf{sFID} $\downarrow$ \\
    \midrule
    AE & 24.80  & 29.90  \\
    DAE & 21.42 & 22.90 \\
    VAE & 32.33 & 32.96 \\
    SD3-VAE & {9.00} & {14.83} \\
    % \midrule
    % \textbf{VMAE (Ours)} & \underline{8.11} & \underline{12.46} \\
    \textbf{VMAE~(Ours)} & \textbf{7.61} & \textbf{9.08} \\
    \bottomrule
    \end{tabular}
\label{tab:imagenet_diffusion_performance}
\end{table}


==> tables/compare_aes.tex <==
%\begin{document}

\begin{table}[t]
    \centering
    \renewcommand{\arraystretch}{1.1}
    % \setlength{\tabcolsep}{8pt}
    \small
    \caption{Comparison of different methods based on reconstruction quality, latent space smoothness, and perceptual compression.
    \label{tab:method_comparison}
    \begin{tabular}{c|ccc}
        \toprule
        Method & Reconstruction & Latent Space & Perceptual \\
        & Quality & Smoothness & Compression \\
        \midrule
        AE   & \tmark & \xmark & \cmark \\
        DAE  & \tmark & \xmark & \cmark \\
        VAE  & \xmark & \cmark & \cmark \\
        SD-VAE & \tmark & \cmark & \tmark \\
        VMAE & \cmark & \cmark & \cmark \\
        \bottomrule
    \end{tabular}
\end{table}

%\end{document}

